Modality-Aware Negative Sampling for Multi-modal Knowledge Graph Embedding

Negative sampling (NS) is widely used in knowledge graph embedding (KGE), which aims to generate negative triples to make a positive-negative contrast during training. However, existing NS methods are unsuitable when multi-modal information is considered in KGE models. They are also inefficient due to their complex design. In this paper, we propose Modality-Aware Negative Sampling (MANS) for multi-modal knowledge graph embedding (MMKGE) to address the mentioned problems. MANS could align structural and visual embeddings for entities in KGs and learn meaningful embeddings to perform better in multi-modal KGE while keeping lightweight and efficient. Empirical results on two benchmarks demonstrate that MANS outperforms existing NS methods. Meanwhile, we make further explorations about MANS to confirm its effectiveness.

==> deleted.tex <==
They can be formally denoted as:
\begin{equation}
    \mathrm{MR}=\frac{1}{2|\mathcal{T}_{test}|}\sum_{i\in\mathcal{T}_{test}}(rank_{ih} +  rank_{it})
\end{equation}

\begin{equation}
    \mathrm{MRR}=\frac{1}{2|\mathcal{T}_{test}|}\sum_{i\in\mathcal{T}_{test}}(\frac{1}{rank_{ih}} +  \frac{1}{rank_{it}})
\end{equation}

\begin{equation}
    \mathrm{Hit@K}=\frac{1}{2|\mathcal{T}_{test}|}\sum_{i\in\mathcal{T}_{test}}
    \mathbf{1}(rank_{ih}\le K) +  \mathbf{1}(rank_{it} \le K)
\end{equation}
where $\mathcal{T}_{test}$ is the test triple set and $rank_{ih}, rank_{it}$ are predicted ranks of head/tail entity prediction for each test triple $i\in\mathcal{T}_{test}$.
